CAMul: Calibrated and Accurate Multi-view Time-Series Forecasting

Probabilistic time-series forecasting enables reliable decision making across many domains. Most forecasting problems have diverse sources of data containing multiple modalities and structures. Leveraging information as well as uncertainty from these data sources for well-calibrated and accurate forecasts is an important challenging problem. Most previous work on multi-modal learning and forecasting simply aggregate intermediate representations from each data view by simple methods of summation or concatenation and do not explicitly model uncertainty for each data-view. We propose a general probabilistic multi-view forecasting framework CAMul, that can learn representations and uncertainty from diverse data sources. It integrates the knowledge and uncertainty from each data view in a dynamic context-specific manner assigning more importance to useful views to model a well-calibrated forecast distribution. We use CAMul for multiple domains with varied sources and modalities and show that CAMul outperforms other state-of-art probabilistic forecasting models by over 25\% in accuracy and calibration.

==> benchmarks.tex <==
\begin{table*}[h]
\centering
\scalebox{0.85}{
\begin{tabular}{l|l|l|l}
Benchmark    & Dataset                                                                                                                                                                                                                                                                & Target                                                                                                          & Views(View type)                                                                                                                                            \\ \hline
\begin{tabular}[c]{@{}l@{}}\texttt{google-symptoms}\\ \cite{googledataset}\end{tabular} & \begin{tabular}[c]{@{}l@{}}Historical wILI sequences and \\ anonymized search volumes for  14 flu-related \\ symptoms for 10 HHS regions and national level.\end{tabular}                                                                                             & \begin{tabular}[c]{@{}l@{}}Future wILI values for each \\  HHS region's sequence\\  at 1- to 4-weeks ahead\end{tabular} & \begin{tabular}[c]{@{}l@{}}Past sequences (Sequence)\\ HHS adjacency (Graph)\\ Months (Static)\end{tabular}                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}\texttt{covid19}\\ \cite{cramer2021evaluation1}\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Weekly data related to Covid-19 surveillance including  \\ from hospital records,  mortality, hospitalization\\ counts,  mobility, exposure and survey data collected  \\ by \cite{kamarthi2021back2future} for 50 US states\end{tabular} & \begin{tabular}[c]{@{}l@{}}Mortality for \\ 50 US states at\\ 1- to 4-weeks ahead\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}Mortality (Sequence)\\ Line-list (Sequence)\\ Mobility (Sequence)\\ Demographics (Static)\\ State adjacency (Graph)\end{tabular} \\ \hline
 \begin{tabular}[c]{@{}l@{}}\texttt{power}\\ \cite{powerdataset} \end{tabular}        & \begin{tabular}[c]{@{}l@{}}Minute-wise Household power consumption\\  measurements for a year with a total of \\ 260,640 measurements each with\\  7 features from 3 meters.\end{tabular}                                                                                          & \begin{tabular}[c]{@{}l@{}}Total active \\ power consumption \\ next minute\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}Past sequence (Sequence)\\ Time-of-day (Static)\\ Month (Static)\end{tabular}                                                    \\ \hline
\begin{tabular}[c]{@{}l@{}}\texttt{tweet}\\ \cite{shi2019state} \end{tabular}       & \begin{tabular}[c]{@{}l@{}}Weekly Tweet topic distribution for tweets \\ related to Covid-19 pandemic with topics\\  extracted using LDA.\end{tabular}                                                                                                                 & \begin{tabular}[c]{@{}l@{}}1-week ahead topic\\ distribution\end{tabular}                                       & \begin{tabular}[c]{@{}l@{}}Past sequence (Sequence)\\ State adjacency (Graph)\\ Month (Static)\\ Demographics (Static)\end{tabular}                        
\end{tabular}
}
\caption{\textit{Description of benchmark tasks: datasets, target and views.}}
\label{tab:bench}
\end{table*}

==> exrelated.tex <==
\section{Additional Related works}

\paragraph{Probabilistic Time-series Forecasting}
Classical methods of time-series forecasting including exponential smoothing, ARIMA-based models \cite{hyndman2018forecasting} focus on univariate time-series with small number of exogenous features and learn model parameters independently for each sequence. 
Vector Auto-regression (VAR) models extend ARIMA based models to multivatiate time series \cite{stock2001vector}.

Deep learning based time-series models \cite{lim2021time} such as RNN, GRU and LSTMs, transformers \cite{vaswani2017attention} have proven useful in modelling for large number of features capturing long-range complex non-linear patterns in sequences. However, these methods are trained for point-prediction tasks. DeepAR \cite{salinas2020deepar} directly models the mean and variance parameters of the forecast distribution using RNN-based architecture. 
Some recent works are inspired from the space-state models to explicitly model the transition and emission components with deep learning modules such as in the case of Deep Markov Models \cite{krishnan2017structured}, and recent Deep State Space models \cite{li2021learning, rangapuram2018deep}. Others introduce stochasticity into state dynamics of recurrent neural networks such as Stochastic RNN \cite{fraccaro2016sequential}, Variational RNN \cite{chung2015recurrent} and State Space LSTM \cite{zheng2017state}. 
%These methods employ stochastic variational Bayes \cite{kingma2013auto} to learn the parameters of the posterior by improving the log likelihood.
Bayesian Neural Networks have also been used to model time-series forecast distributions \cite{zhu2017deep} but require assigning useful priors to parameters and comes with high computational cost of learning.

Neural Process (NP)~\cite{garnelo2018neural} models a global latent variable for entire dataset to capture uncertainty with is used with input data's embedding to model the distribution parameters. Recurrent neural Process \cite{qin2019recurrent} leverages NP for sequence data. Functional Neural Process (FNP) captures stochastic correlations between input data and datapoints from training distribution to provide a flexible non-parametric mechanism to model output distribution using related training data points in functional space. EpiFNP \cite{kamarthi2021doubt} leveraged this flexible modelling towards sequential data to propose a epidemic forecasting model on univariate sequences for state-of-art calibration and uncertainty.
In contrast, our work leverages FNP for uncertainty modelling of each of the individual views and then \model jointly model the total uncertainty by carefully combining distributions from different views towards a well-calibrated final output distribution.

\paragraph{Multi-view time-series forecasting}

Extracting useful information from multiple data sources and data modalities for enriching prediction models has been a very important machine learning problem with challenges that include
noisy data sources, integrating information from multiple sources and handling different levels of uncertainty and reliability.
Recent advances is deep learning architectures has allowed us to extract representations from variety of data sources such as images \cite{li2016survey}, sequences \cite{salehinejad2017recent}, graphs \cite{hamilton2020graph}, etc, and combine these modules' representation for training in a end-to-end fashion.
In order to integrate these methods most methods employ simple summation or concatenation methods \cite{yan2021deep, li2018survey}. For instance DeepCovidNet \cite{ramchandani2020deepcovidnet} uses spatio-temporal and static features using simple summation for Covid-19 prediction. \citet{ekambaram2020attention} similarly integrate images, text and static features for predicting consumer sales.

Moreover, most of these methods do not focus on probabilistic forecasting unlike \cite{chen2021unite} which uses  EHR sequence data, static demographic and location data and learn a data-source specific weight by pre-training the aggregated embeddings on prediction task of deciding if patient requires a treatment. Then, they employ a Gaussian Process approach to learn forecast probability on these embeddings to capture uncertainty.

In contrast, we model data-view specific and modality specific uncertainty by learning a latent distribution for each view which allows the model to reason about data reliability, source specific uncertainty and inherent noise when it integrates uncertainty-aware stochastic representations of all views towards the final forecast distribution.



==> table1_1.tex <==
\begin{table*}[!th]
\centering
\scalebox{0.85}{
\begin{tabular}{lccc|lccc}
            & \multicolumn{3}{c|}{\texttt{covid19}}                                           &              & \multicolumn{3}{c}{\texttt{google-symptoms}}                                        \\
            & CRPS                 & CS                     & IS                     &              & CRPS                   & CS                     & IS                    \\ \hline
SARIMA      & 61 $\pm$ 3.40            & 0.42 $\pm$ 0.017          & 6.32 $\pm$ 0.042          & SARIMA       & 1.14 $\pm$ 0.017          & 0.43 $\pm$ 0.008          & 3.11 $\pm$ 0.240          \\
DeepAR      & 32.6 $\pm$ 6.40          & 0.19 $\pm$ 0.015          & 2.21 $\pm$ 0.015          & DeepAR       & 0.55 $\pm$ 0.013          & 0.14 $\pm$ 0.003          & 1.42 $\pm$ 0.130          \\
DSSM        & 49.6 $\pm$ 3.10          & 0.22 $\pm$ 0.009          & 2.13 $\pm$ 0.041          & DSSM         & 0.52 $\pm$ 0.011          & 0.13 $\pm$ 0.003          & 2.11 $\pm$ 0.140          \\
RNP         & 51.2 $\pm$ 7.60          & 0.35 $\pm$ 0.018          & 4.33 $\pm$ 0.031          & RNP          & 0.71 $\pm$ 0.047          & 0.43 $\pm$ 0.006          & 4.13 $\pm$ 0.150          \\
GP          & 25.2 $\pm$ 1.10          & 0.27 $\pm$ 0.012          & 3.19 $\pm$ 0.015          & GP           & 0.68 $\pm$ 0.021          & 0.21 $\pm$ 0.008          & 1.87 $\pm$ 0.410          \\
GraphDF-RBF & 31.4 $\pm$ 2.80          & 0.21 $\pm$ 0.017          & 2.75 $\pm$ 0.046          & GraphDF- RBF & 0.59 $\pm$ 0.016          & 0.08 $\pm$ 0.002          & 1.03$\pm$ 0.240           \\
GraphDF-Adj & 37.6 $\pm$ 3.30          & 0.28 $\pm$ 0.013          & 2.44 $\pm$ 0.017          & GraphDF- Adj & 0.64 $\pm$ 0.057          & 0.08 $\pm$ 0.005          & 2.87 $\pm$ 0.610          \\ \hline
DeepCovid   & 30.5 $\pm$ 7.10          & 0.18 $\pm$ 0.011          & 3.41 $\pm$ 0.029          & EpiDeep      & 0.93 $\pm$ 0.046          & 0.24 $\pm$ 0.007          & 4.26 $\pm$ 0.910          \\
CMU-TS      & 21.8 $\pm$ 4.80          & \textbf{0.14 $\pm$ 0.015} & 3.17 $\pm$ 0.064          & EpiFNP       & 0.31 $\pm$ 0.051          & \textbf{0.04 $\pm$ 0.002} & \textbf{0.56 $\pm$ 0.180} \\ \hline
\model       & \textbf{17.4 $\pm$ 5.40} & \textbf{0.15 $\pm$ 0.007} & \textbf{1.42 $\pm$ 0.017} & \model        & \textbf{0.24 $\pm$ 0.060} & \textbf{0.04 $\pm$ 0.004} & \textbf{0.43 $\pm$ 0.020} \\ \hline
\model-C     & \textbf{18$\pm$3.10}     & 0.19$\pm$0.003            & 1.73$\pm$0.024            & \model-C      & 0.29$\pm$0.022            & 0.05 $\pm$ 0.001          & \textbf{0.48 $\pm$ 0.060} \\
\model-S     & \textbf{18.4$\pm$2.90}   & 0.15$\pm$0.007            & 1.64 $\pm$ 0.037          & \model-S      & 0.31$\pm$0.064            & 0.04$\pm$0.006            & \textbf{0.46$\pm$0.020}   \\
\model-D     & 27.3$\pm$7.10            & 0.31$\pm$0.012            & 3.26 $\pm$0.021           & \model-D      & 0.74$\pm$0.081            & 0.19$\pm$0.002            & 1.83$\pm$0.040           
\end{tabular}
}

\caption{Evaluation scores for \model and other baselines for \texttt{covid19} and \texttt{google-symptoms} benchmarks. The best performing model's (\model's) score and scores that are not significantly worse are shown in bold.}
\label{tab:metrics2}
\end{table*}



==> table2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|r|r|rr}
                     & \multicolumn{2}{c|}{Power consumption}              & \multicolumn{2}{c}{Tweet topics}                            \\ \hline
                     & \multicolumn{1}{l|}{CRPS} & \multicolumn{1}{l|}{IS} & \multicolumn{1}{l|}{CRPS}          & \multicolumn{1}{l}{IS} \\ \hline
{\ul View selection} & \textbf{0.46}             & \textbf{0.93}           & \multicolumn{1}{r|}{\textbf{0.59}} & \textbf{0.82}          \\
{\ul Concat}         & 1.13                      & 2.88                    & \multicolumn{1}{r|}{1.06}          & 1.15                   \\ \hline
                     & \multicolumn{2}{c|}{Covid-19}                       & \multicolumn{2}{c}{Flu wILI}                                \\ \hline
{\ul View selection} & \textbf{1.74}             & \textbf{1.42}           & \multicolumn{1}{r|}{\textbf{0.24}} & \textbf{0.43}          \\
{\ul Concat}         & 1.8                       & 2.66                    & \multicolumn{1}{r|}{0.29}          & 0.48                  
\end{tabular}
\caption{Comparison of CRPS scores with and without view selection}
\label{tab:select}
\end{table}
